Skein theories for virtual tangles

In this paper, we use skein-theoretic techniques to classify all virtual knot polynomials and trivalent graph invariants with certain smallness conditions. The first half of the paper classifies all virtual knot polynomials giving non-trivial invariants strictly smaller than the one given by the Higman-Sims spin model. In particular, we exhibit a family of skein theories coming from $\text{Rep}(O(2))$ with an interesting braiding. In addition, all skein theories of oriented virtual tangles with some smallness conditions are classified. In the second half of the paper, we classify all non-trivial invariants of (perhaps non-planar) trivalent graphs coming from symmetric trivalent categories. For each of these categories, we also classify when the sub-category generated by only the trivalent vertex is braided. An interesting example of this arise from the tensor category Deligne's $S_t$.

==> diagrams/tikz/cupcapstrand.tex <==
\begin{tikzpicture}[baseline={([yshift=-.5ex]current bounding box.center)}, scale = .5]
	\draw (.1,-.5) to[out = 90, in = 0] (-.2,-.1) to[out = 180, in = 90] (-.5,-.5);
    \draw (.1,.5) to[out = -90, in = 0] (-.2,.1) to[out = 180, in = -90]  (-.5,.5);
    \draw (.4,-.5) -- (.4,.5);
\end{tikzpicture}

==> text/Background.tex <==
The following definitions are were given in \cite{Jon99} (See also \cite{Pet09}): 

\subsection{Definition of a planar algebra}

\begin{definition}
A planar diagram is described as follows. The diagram is the unit disc $\mathcal{D}$ with a finite number of clockwise-numbered boundary points. In addition, there are a finite number of internal discs each with their own finite number of clockwise-numbered boundary points. The boundary points of all diagrams are paired by smooth, non-crossing curves called the strings of the diagram. In addition, there may also be a finite number of closed strings not connecting to any discs. The strings lie between the internal discs and $\mathcal{D}$, and the connected components of the interior minus the strings are called the regions of the planar diagram. To indicate the first point on the boundary of the external or an internal disc, the region immediately preceding it is starred near the relevant boundary component. 
\end{definition}
%
An example of a planar diagram is
%
\begin{equation}\label{eq:paex}
\includegraphics[valign = c, scale = .7]{diagrams/pdf/Tangle.pdf}
\end{equation}
%
Because of the appearance of these diagrams, they are often called ``spaghetti and meatball" diagrams. We can compose diagrams $A$ and $B$ if the number of strands connecting to the outer disc of $B$ is equal to the number of strands connecting to one of the inner discs of $A$ or vice versa. An example of this composition is below:
%
\begin{equation}\label{comp}
\includegraphics[valign = c, scale = .7]{diagrams/pdf/Composition.pdf}
\end{equation}
%
In this example, the planar diagram with inner disc 4 is inserted into inner disc 2 of the other planar diagram, giving the new planar diagram on the right.  
%
\begin{definition}
The planar operad, $\mathcal{P},$ is the set of isotopy classes of planar diagrams under composition as described above.  
\end{definition}
% 
\begin{definition}
The standard involution of a planar diagram is performed in the following steps. Take any diameter of the outer disc through the starred region. Reflect the diagram over that diameter. Finally, relabel all inner and outer boundary points so that the original starred regions of each disc are preserved.
\end{definition}
%
As an example, consider 
%
\begin{equation*}
\includegraphics[valign = c, scale = .7]{diagrams/pdf/Tangle.pdf} ~~ \overset{*}{\longrightarrow} \includegraphics[valign = c, scale = .7]{diagrams/pdf/Reflection.pdf}
\end{equation*}
%
Taking an involution can be quite cumbersome for large planar diagram. As a solution, we draw the diagrams in what is often called ``standard'' form.
%
\begin{definition}\label{def:std}
A planar diagram $T$ is drawn in \emph{standard form} if the input and output circles are drawn as rectangles, with strings attached only to the top or bottom and the starred region represented by the left-hand side of the rectangle.
\end{definition}
%
By drawing planar diagrams in this way, an involution simply rotates the planar diagram 180 degrees but takes the complex conjugate of any coefficients. In what follows, all planar diagrams are assumed to be in standard form unless explicitly drawn otherwise.
%
\begin{definition}
A planar algebra is a family of $\mathbbm{k}$-vector spaces $\mathcal{V}=\{V_0,V_1,V_2,\dots\},$ together with an action of the planar operad. This action assigns a multilinear map to every $T\in\mathcal{P}$ that respects the composition of planar diagrams. Moreover, if $T$ is a planar diagram with $k$ inner discs, the corresponding multilinear map is
%
\begin{equation*}
T:V_{i_1}\otimes V_{i_2}\otimes\dots\otimes V_{i_k} \to V_o
\end{equation*}
%
so that $i_m$ is the number of strands connected to the boundary of the $m$-th inner boundary disc, and $o$ is the number of strands connected to the outer boundary disc. $\mathcal{V}$ is a planar $\ast$-algebra if in addition the action of the planar operad also respects the involution on $\mathcal{P}.$
\end{definition}
%
Put another way, a planar algebra is a graded vector space that respects the action of the planar operad. In this paper we will assume that $\mathbbm{k} = \mathbb{C}$. The dimension of a planar algebra is usually given by a sequence $a_0,a_1,a_2,\dots$ where $a_i = \dim(V_i)$ and $V_i$ is often called the $i$-box space. 

The planar operad can be thought of as the set of operations on a planar algebra. In (\ref{eq:paex}), for example, a planar algebra would determine a multilinear map
%
\begin{equation*}
V_2 \otimes V_4 \otimes V_4 \to V_6
\end{equation*}
%
Some of these operations appear often and have common names, shown below for two elements of a planar algebra $X$ and $Y$: 
%
\begin{center}
\begin{tabular}{ll}
\emph{Multiplication of two diagrams:}
 &
$\input{diagrams/tikz/Multiplication.tex}$
 \\
 \\
\emph{Capping off a diagram on the top:} 
&
$\input{diagrams/tikz/Capping.tex}$
\\
\\
\emph{Rotating a diagram by ``1 click:''}
&
$\input{diagrams/tikz/Rotating.tex}$
\end{tabular}
\end{center}
%
Of course, we might also want to cap a diagram off in some other way or rotate by more than 1 click, both of which are defined similarly. Note that multiplication is only defined if the number of bottom endpoints for $Y$ is the same as the number of top endpoints of $X$.
%
\begin{definition}\label{def:modulus}
Let $\mathcal{V}$ be a planar algebra and $f$ be the multilinear map associated with some planar diagram $T$. Then $\mathcal{V}$ is said to have modulus $d$ if for all $T \in\mathcal{P}$ inserting a closed string into $T$ is equivalent to the map $d\cdot f,$ for some $d \in\mathbbm{k}^\times.$    
\end{definition}
%
Alternatively, one can think of a planar algebra having modulus $d$ if there exists as relation of the form:
%
\begin{equation*}
    \skeincircle ~=~ d
\end{equation*}
%
where the right-hand side of the equation is $d$ times the diagram with no strings, called the empty diagram. For this reason, we often call $d$ the circle parameter. 

\begin{definition}
A planar algebra $\mathcal{V}$ is called \emph{evaluable} if $\dim V_0 = 1$, or, equivalently, any element of $V_0$ is equivalent to the empty diagram up to a scalar. 
\end{definition}

Thus we can define a map from $V_0\to\mathbbm{k}$ by sending the empty diagram to 1. This map can be used to define an inner product on each $V_n.$

\begin{definition}
Let $\mathcal{V}$ be an evaluable planar algebra. We define an inner product on $\mathcal{V}$ as
%
\begin{center}
$\input{diagrams/tikz/trace.tex}$
\end{center}
%
\end{definition}

Notice that this definition requires that if $X$ has $n$ top strands and $m$ bottom strands then $Y$ must have $m$ top strands and $n$ bottom strands. We would like to be able to calculate an inner product for any $V_n$, regardless of whether this condition holds. If $\mathcal{V}$ is planar $\ast$-algebra however, note that $Y^\ast$ will always exist and satisfy these requirements. As such, sometimes $Y^\ast$ is used instead of $Y$ for planar $\ast$-algebras. Of course, we could have also connected the strands on the left. If they are the quantities are the same, the planar algebra is said to be \emph{spherical}.

\begin{definition}
An element $v_n\in V_n$ that has the property that $<\!v_n,w_n\!> ~= 0$ for all $w_n\in V_n$ is called a negligible element. 
\end{definition}

\begin{definition}\label{degenerate}
We say that a planar algebra is \emph{non-degenerate} if it has no negligible elements.
\end{definition}

How does one find all negligible elements of $V_n?$ Given a basis for $V_n$, $\{v_1,v_2,\dots,v_k\}$, we can take the matrix of inner products, $M$, where  the $(i,j)$-th entry of $M$ is the inner product of $v_i$ and $v_j.$ The null space of this matrix would then give us the linear subspace of $V_n$ spanned by the negligible elements.

We now recall the definition of a rotational eigenvector in the style of \cite{Jon01}:
%
\begin{definition}\label{def:eigen}
A rotational eigenvector is a diagram $S$ such that if $\rho$ is the planar diagram that rotates the diagram one click then $\rho(S)=\zeta\cdot S,$ for some $\zeta\in\mathbb{C}.$
\end{definition}
%
If $\rho$ has $n$ output strands, we note that this immediately implies that $\zeta$ is an $n$-th root of unity, as $\zeta^n S =\rho^n(S) = S$. Because this space of relations is a $\mathbb{Z}/n\mathbb{Z}$ representation, the action is diagonalizable. Thus, given that $\rho^n(S) = S$ we know that $\rho(S) = \zeta\cdot S.$ 

Because we will be focusing on classifying planar algebras, we define the notion of subplanar algebra, quotient planar algebra, and isomorphism:
%
\begin{definition}
$\mathcal{W}$ is a subplanar algebra of $\mathcal{V}$ if $W_i \subseteq V_i$ for all $i$ and if the inclusion maps $\{i_k:W_k \to V_k\}$ intertwine the actions of the planar operad.

\end{definition}
%
\begin{definition}
$\mathcal{Q}$ is a quotient of a planar algebra $\mathcal{V}$ if $Q_i$ is a quotient of $V_i$ and if the quotient maps $\{\pi_k:V_k \to Q_k\}$ intertwine the actions of the planar operad.
\end{definition}
%
\begin{definition}
Two planar algebras $\mathcal{V}$ and $\mathcal{W}$ are isomorphic if there is a collection of isomorphisms $\{\phi_k:V_k \to W_k\}$ that intertwine the actions of the planar operad. When the planar algebras are $\ast$-planar algebras, we also require that the isomoprhism be a $\ast$-isomorphism. 
\end{definition}


\subsection{Skein Theories}

When one studies all quotients of a ring or algebra, one might instead classify all two-sided ideals. Similarly, when studying the quotients of a planar algebra, we instead classify all its \emph{planar} ideals.

\begin{definition}
Let $\mathcal{V}$ be a planar algebra. A planar ideal, $\mathcal{I}$, is a subset of $\mathcal{V}$ such that $\mathcal{I}$ is the kernel of some quotient map of $\mathcal{V}.$ 
\end{definition}

Equivalently, $\mathcal{I}$ is a planar ideal if it is closed under arbitrary composition with any element of the planar algebra. That is, if we let $T$ be any planar tangle, then $T(v_1, \dots, v_k)\in\mathcal{I}$ if at least one $v_i$ is an element of $\mathcal{I}$ for all possible choices of the other elements. Just like a two-sided ideal in a ring, a planar ideal can also be written using relations, which we call skein relations.
%
\begin{definition}
Let $\mathcal{V}$ be a planar algebra. A \emph{skein relation} is an element of the kernel of a quotient map from $\mathcal{V}$.  A \emph{skein theory} is a set of skein relations that generates a planar ideal.
\end{definition}
%
Thus, giving a skein theory would be an equivalent way of defining a quotient of a planar algebra. If we wanted to classify all quotients of a planar algebra, then, we could instead classify all skein theories of that planar algebra. In the next section, we will examine a number well-known examples of skein theories.
